Low-light Image and Video Enhancement via Selective Manipulation of Chromaticity

Image acquisition in low-light conditions suffers from poor quality and significant degradation in visual aesthetics. This affects the visual perception of the acquired image and the performance of various computer vision and image processing algorithms applied after acquisition. Especially for videos, the additional temporal domain makes it more challenging, wherein we need to preserve quality in a temporally coherent manner. We present a simple yet effective approach for low-light image and video enhancement. To this end, we introduce "Adaptive Chromaticity", which refers to an adaptive computation of image chromaticity. The above adaptivity allows us to avoid the costly step of low-light image decomposition into illumination and reflectance, employed by many existing techniques. All stages in our method consist of only point-based operations and high-pass or low-pass filtering, thereby ensuring that the amount of temporal incoherence is negligible when applied on a per-frame basis for videos. Our results on standard lowlight image datasets show the efficacy of our algorithm and its qualitative and quantitative superiority over several state-of-the-art techniques. For videos captured in the wild, we perform a user study to demonstrate the preference for our method in comparison to state-of-the-art approaches.

==> cutouts.tex <==
\iffalse 
\begin{figure} [tb]
	%\centering%
	\subfigure[Input image]{%
		\begin{tikzpicture}
		\node{
		\includegraphics[width=0.325\columnwidth]{resources/teaser/input.png}};%
		\end{tikzpicture}
		\label{fig:teaser_input}%
	}\hfill
	\subfigure[LIME~\shortcite{LIME_Guo2017}]{%
		\includegraphics[width=0.325\columnwidth]{resources/teaser/out_LIME.png}%
		\label{fig:teaser_LIME}%
	}\hfill
	\subfigure[Zero-DCE~\shortcite{Zero_DCE_Guo2020}]{%
		\includegraphics[width=0.325\columnwidth]{resources/teaser/out_ZeroDCE.png}%
		\label{fig:teaser_MBLLEN}%
	}\\%[-2ex]
	\subfigure[LLVE~\shortcite{Zhang_Temporal2021}]{%
		\includegraphics[width=0.325\columnwidth]{resources/teaser/out_StableLLVE.png}%
		\label{fig:teaser_LLVE}%
	}\hfill
	\subfigure[Ours]{%
		\includegraphics[width=0.325\columnwidth]{resources/teaser/out_ours_new.png}%
		\label{fig:teaser_Ours}%
	}\hfill
	\subfigure[Ground Truth]{%
		\includegraphics[width=0.325\columnwidth]{resources/teaser/out_gt.png}%
		\label{fig:teaser_GT}%
	}
	\caption{Comparison of low-light image enhancement for two image-based (b and c) and one video based (d) method. Ours (e) is able to brighten image while preserving details and avoiding artifacts in terms of noise and color shifts.}%
	\label{fig:teaser}
\end{figure}
\fi 

\iffalse 
- What Color Space to compute intensity and why?
+ We take the "Y" channel of the YCbCr space as intensity. Efficient to compute and is effective in perceptual editing.
- Why not using perceptual L*a*b?
- Open Question: Why is chromaticity is so bright?
+ Get rid of multiplicative lighting effects, thereby significantly getting rid of shadows and shading. Moreover, the normalization makes the pixel color more saturated thereby making it look bright.  
- Why do not perform gamma correction on input image instead of the virtual exposure series?
+ Performing gamma correction before makes the result more noisy.
- Discuss different scaling functions (linear, non-linear) and their impact for detail layers
- Virtual Exposure series: how to determine $\alpha_1, \ldots \alpha_n$ and  $\gamma_1, \ldots \gamma_n$  based on a single parameters $\alpha$?
- What are minimum required pyramid levels?
+ Min. - 2, however the results miss fine details. Level of 4 or 5 gives a good trade-off between performance and quality.
- What is the difference between to: %https://people.csail.mit.edu/sparis/publi/2011/siggraph/Paris_11_Local_Laplacian_Filters.pdf
- Performance tests with state-of-the-art spatial resolution (HD, FullHD, 4K, ...)
- What is the overhead of CUDA state changes (since we have a multi-stage pipeline
- Please compute comparison video for alternative approaches
- Metric for low-light enhancement (image/spatial vs. video/spatio-temporal)?
- Video: 60 FPS vs. 24 FPS
- Method close to Unsharp Masking 
- 
* Motivate/Justify: why using chromaticity? Are there alternatives? 
	-> Choice influences the noise -> which we want to get rid of
* L*a*b for Lumincance Intensity
* What is the difference to linear interpoaltion between I and C(I)
-> Can this be formulated as loss function? If yes, low resolution only due to limitation of ML
* Difference to exposure fusion: no additional information in virtual exposure series
* Please test with 720p and 1080p
* Application to Video HQ, LS -> Export | LQHS -> Preview
\fi 


\iffalse 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Fig: Virtual Exposure Sequence
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure} [tb]
%\centering%
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 1.0$ and $\alpha = 0.01$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_1_0/a_0_01.png}%
	\label{fig:g_1_0_a_0_01}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 1.0$ and $\alpha = 0.05$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_1_0/a_0_05.png}%
	\label{fig:g_1_0_a_0_05}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 1.0$ and $\alpha = 0.15$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_1_0/a_0_15.png}%
	\label{fig:g_1_0_a_0_15}%
\end{subfigure}\\[-1.5ex]
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.5$ and $\alpha = 0.01$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_5/a_0_01.png}%
	\label{fig:g_0_5_a_0_01}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.5$ and $\alpha = 0.05$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_5/a_0_05.png}%
	\label{fig:g_0_5_a_0_05}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.5$ and $\alpha = 0.15$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_5/a_0_15.png}%
	\label{fig:g_0_5_a_0_15}%
\end{subfigure}\\[-1.5ex]
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.25$ and $\alpha = 0.01$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_25/a_0_01.png}%
	\label{fig:g_0_25_a_0_01}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.25$ and $\alpha = 0.05$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_25/a_0_05.png}%
	\label{fig:g_0_25_a_0_05}%
\end{subfigure}\hfill
\begin{subfigure}{0.327\columnwidth}%
	\subcaption{$\gamma = 0.25$ and $\alpha = 0.15$}%
	\includegraphics[width=\columnwidth]{resources/exposure_sequence/g_0_25/a_0_15.png}%
	\label{fig:g_0_25_a_0_15}%
\end{subfigure}\\[-1.5ex]
\caption{\textit{Virtual exposure sequence} for the input image in \Cref{fig:teaser}: as a sequence of \acp{AC} generated by varying values of $\alpha$ and $\gamma$.}%
\label{fig:exposure_sequence}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi 

%For being self contained we describe the exposure-fusion method in detail.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\paragraph{Exposure Fusion}


\iffalse 
\begin{table}[tb]
	\label{RL:Tab:quant_eval}
	\caption{Quantitative evaluation of different methods on the test data of LOL~\cite{Deep_Ret_Wei2018} dataset. The best method is shown in \textcolor{red}{red} and the next best in \textcolor{blue}{blue}. }
	\begin{tabular}{|l|l|l|l|}
		\hline
		Method     & PSNR ($\uparrow$)                      & SSIM ($\uparrow$)                     & MAE ($\downarrow$)                    \\ \hline
		LIME       & 16.903                                 & 0.591                                 & 0.132                                 \\ \hline
		SRIE       & 13.877                                 & 0.658                                 & 0.208                                 \\ \hline
		MBLLEN     & \textcolor{blue}{ \textbf{17.858}} & \textcolor{blue}{ \textbf{0.698}} & \textcolor{blue}{ \textbf{0.123}} \\ \hline
		RetinexNet & 14.977                                 & 0.405                                 & 0.160                                 \\ \hline
		LLVE       & 17.364          & 0.672                                 & 0.127                                 \\ \hline
		Zero-DCE   & 14.861                                 & 0.585                                 & 0.185                                 \\ \hline
		Ours       & \textcolor{red} {\textbf{19.272}} & \textcolor{red} { \textbf{0.710}} & \textcolor{red} { \textbf{0.109}} \\ \hline
	\end{tabular}
\end{table}
\fi 

\iffalse 
The above measures are quantified using a scalar-valued weight map for each input image in the sequence.
Final well-exposed image is obtained by weighted blending of all input images with a multi-scale pyramid technique.

An image in the exposure sequence can potentially contain large over-/under-exposed regions that do not contain valuable visual information and thus should get less weight.
On the other hand, visually interesting areas containing more details should get a higher weight.
To achieve the above, the following measures are used.

\begin{description} 
%%
%%
\item[Contrast:] An efficient way to measure the amount of image- texture/details is by computing the Laplacian magnitude of the grayscale version of the image. 
We consider the image intensity $\mathit{In}(I)$(\Cref{RL:Eqn:Chroma}) as its grayscale version and the per-pixel $\bm{x}$ weight is given as
%%
\begin{equation}
c_k(\bm{x}) = \left|\Delta \mathit{In}(E_k)(\bm{x})\right|,
\end{equation} 
where $\Delta$ stands for Laplacian operator.

%%
%%
\item[Saturation:] Saturated colours are a desirable characteristic for the final image, as they make the image appear vivid. 
Saturation, for each pixel, is efficiently measured by the standard deviation within the RGB color channels. 
Thus the per-pixel saturation weight is given as
%%
\begin{equation}
s_k(\bm{x}) = \sqrt{\frac{\underset{Ch \in r,g,b}{\sum}{\left({Ch}_k(\bm{x}) - \mu_k(\bm{x})\right)}^2 }{3}},
\end{equation} 
%%
where $\mu_k(\bm{x})$ is the mean of individual color channels.
%%
%%
\item[Well-exposedness:] This weight determines whether the given pixel is under-/over-exposed. 
Gaussian-based weighting, for each $R$, $G$, and $B$ color channel, is designed in a manner where less weight is assigned to under-/over-exposed pixels. 
Thus, the per-pixel well-exposedness weight is given as
%%
\begin{equation}
e_k(\bm{x}) = \underset{{Ch} \in r,g,b}{\prod} exp\left(\frac{-{({Ch}_k(\bm{x}) - 0.5)}^2}{2\sigma^2}\right),
\end{equation} 
%%
where $\sigma$ is a free parameter.
\end{description}
\fi 






\iffalse 
\begin{algorithm}
	\label{RL:alg:low-quality}
	\DontPrintSemicolon
	
	\KwInput{Input Image $I$, Adaptivity parameter $\alpha$, Gamma correction parameter $\gamma$ }
	\KwOutput{Enhanced Output $O$}
	Compute $A_c$ (using \Cref{eqn:adap_chroma})   \;
	$tmp = {(A_c)}^{\gamma}$ \tcp*{gamma correction}
	$O = Denoise(tmp)$ \;
	\caption{Low-Quality and Fast}
\end{algorithm}
\fi 






\iffalse 
\begin{algorithm}
	\DontPrintSemicolon
	
		\If{$i \equiv 0(mod4)$} {
		%\State
		$temp = SUBWORD(ROTWORD(temp))\oplus RCon[i/4]$\;
	}%\EndIf
	$w[i] \leftarrow w[i-4] \oplus temp$\;
	
	\KwInput{Your Input}
	\KwOutput{Your output}
	\KwData{Testing set $x$}
	$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
	\tcc{Now this is an if...else conditional loop}
	\If{Condition 1}
	{
		Do something    \tcp*{this is another comment}
		\If{sub-Condition}
		{Do a lot}
	}
	\ElseIf{Condition 2}
	{
		Do Otherwise \;
		\tcc{Now this is a for loop}
		\For{sequence}    
		{ 
			loop instructions
		}
	}
	\Else
	{
		Do the rest
	}
	
	\tcc{Now this is a While loop}
	\While{Condition}
	{
		Do something\;
	}
	
	\caption{Example code}
\end{algorithm}
\fi 
